The Most Metal-Poor Stars. III. The Metallicity Distribution Function and CEMP Fraction

We examine the metallicity distribution function (MDF) and fraction of carbon-enhanced metal-poor (CEMP) stars in a sample that includes 86 stars with [Fe/H] < -3.0, based on high-resolution, high-S/N spectroscopy, of which some 32 objects lie below [Fe/H] = -3.5. After accounting for the completeness function, the "corrected" MDF does not exhibit the sudden drop at [Fe/H] = -3.6 that was found in recent samples of dwarfs and giants from the Hamburg/ESO survey. Rather, the MDF decreases smoothly down to [Fe/H] = -4.1. Similar results are obtained from the "raw" MDF. We find the fraction of CEMP objects below [Fe/H] = -3.0 is 23 +/- 6% and 32 +/- 8% when adopting the Beers et al. and Aoki et al. CEMP definitions, respectively. The former value is in fair agreement with some previous measurements, which adopt the Beers et al. criterion.

==> tab1.tex <==
\begin{deluxetable}{lrrrrrrrrrr}
\tabletypesize{\scriptsize}
\tablecolumns{9} 
\tablewidth{0pc} 
\tablecaption{Stellar Parameters and Carbon Abundance \label{tab:param}}
\tablehead{ 
\colhead{Star} & 
\colhead{RA2000\tablenotemark{a}} &
\colhead{DEC2000\tablenotemark{a}} &
\colhead{\teff} & 
\colhead{$\log g$} & 
\colhead{$\xi_t$} & 
\colhead{[M/H]$_{\rm model}$} & 
\colhead{[Fe/H]$_{\rm derived}$} & 
\colhead{[C/Fe]\tablenotemark{b}} & 
\colhead{C-rich\tablenotemark{c}} & 
\colhead{Source} \\
\colhead{} & 
\colhead{} &
\colhead{} &
\colhead{(K)} & 
\colhead{(cgs)} & 
\colhead{(\kms)} & 
\colhead{} & 
\colhead{} & 
\colhead{} \\
\colhead{(1)} & 
\colhead{(2)} &
\colhead{(3)} &
\colhead{(4)} & 
\colhead{(5)} & 
\colhead{(6)} & 
\colhead{(7)} & 
\colhead{(8)} & 
\colhead{(9)} & 
\colhead{(10)} &
\colhead{(11)} 
}
\startdata 
CS29527-015 &  00 29 10.7 & $-$19 10 07.2 & 6577 & 3.89 & 1.9 & $-$3.3 & $-$3.32 & 1.18 & 1 &   5 \\
CS30339-069 &  00 30 16.0 & $-$35 56 51.2 & 6326 & 3.79 & 1.4 & $-$3.1 & $-$3.05 & 0.56 & 0 &   5 \\
CS29497-034 &  00 41 39.8 & $-$26 18 54.4 & 4983 & 1.96 & 2.0 & $-$3.0 & $-$3.00 & 2.72 & 1 &   4 \\
HD4306 &  00 45 27.2 & $-$09 32 39.9 & 4854 & 1.61 & 1.6 & $-$3.1 & $-$3.04 & 0.11 & 0 &  12 \\
CD-38 245 &  00 46 36.2 & $-$37 39 33.5 & 4857 & 1.54 & 2.2 & $-$4.2 & $-$4.15 & $<-$0.33 & 0 &   7 \\
HE0049-3948 &  00 52 13.4 & $-$39 32 36.9 & 6466 & 3.78 & 0.8 & $-$3.7 & $-$3.68 & <1.81 & 0 &   1 \\
HE0057-5959 &  00 59 54.0 & $-$59 43 29.9 & 5257 & 2.65 & 1.5 & $-$4.1 & $-$4.08 & 0.86 & 1 &   1 \\
HE0102-1213 &  01 05 28.0 & $-$11 57 31.1 & 6100 & 3.65 & 1.5 & $-$3.3 & $-$3.28 & <1.31 & 0 &   1 \\
CS22183-031 &  01 09 05.1 & $-$04 43 21.1 & 5202 & 2.54 & 1.1 & $-$3.2 & $-$3.17 & 0.42 & 0 &  12 \\
HE0107-5240 &  01 09 29.2 & $-$52 24 34.2 & 5100 & 2.20 & 2.2 & $-$5.3 & $-$5.54 & 3.85 & 1 &   8 \\
CS29518-043 &  01 18 38.3 & $-$30 41 02.7 & 6550 & 4.29 & 1.5 & $-$3.2 & $-$3.14 & \ldots & 0 &   5 \\
HE0130-2303 &  01 33 18.2 & $-$22 48 36.8 & 6548 & 4.28 & 1.5 & $-$3.0 & $-$3.02 & \ldots & 0 &   6 \\
HE0132-2439 &  01 34 58.9 & $-$24 24 18.6 & 5249 & 2.63 & 1.6 & $-$3.8 & $-$3.79 & 0.62 & 0 &   6, 10 \\
53327-2044-515\tablenotemark{d} &  01 40 36.2 & +23 44 58.1 & 5703 & 4.68 & 0.8 & $-$4.0 & $-$4.00 & 1.13 & 1 &   1 \\
53327-2044-515\tablenotemark{e} &  01 40 36.2 & +23 44 58.1 & 5703 & 3.36 & 1.5 & $-$4.1 & $-$4.09 & 1.57 & 1 &   1 \\
HE0146-1548 &  01 48 34.7 & $-$15 33 24.4 & 4636 & 0.99 & 2.1 & $-$3.5 & $-$3.46 & 0.84 & 1 &   1 \\
HE0148-2611 &  01 50 59.6 & $-$25 57 03.2 & 6605 & 4.23 & 1.3 & $-$3.1 & $-$3.05 & \ldots & 0 &   6 \\
HE0218-2738 &  02 21 03.9 & $-$27 24 40.5 & 6593 & 4.29 & 1.5 & $-$3.6 & $-$3.57 & \ldots & 0 &   6 \\
HE0228-4047\tablenotemark{d} &  02 30 33.7 & $-$40 33 54.8 & 6515 & 4.35 & 1.6 & $-$3.8 & $-$3.75 & <1.88 & 0 &   1 \\
HE0228-4047\tablenotemark{e} &  02 30 33.7 & $-$40 33 54.8 & 6515 & 3.80 & 1.7 & $-$3.8 & $-$3.75 & <1.98 & 0 &   1 \\
HE0231-6025 &  02 32 30.6 & $-$60 12 11.2 & 6437 & 4.36 & 1.8 & $-$3.1 & $-$3.10 & <1.64 & 0 &   1 \\
CS22189-009 &  02 41 42.4 & $-$13 28 10.5 & 4944 & 1.83 & 1.9 & $-$3.5 & $-$3.48 & 0.31 & 0 &   7 \\
HE0242-0732 &  02 45 00.7 & $-$07 19 42.1 & 6572 & 4.29 & 1.9 & $-$3.3 & $-$3.30 & \ldots & 0 &   6 \\
HE0253-1331 &  02 56 06.7 & $-$13 19 27.0 & 6474 & 4.34 & 1.5 & $-$3.0 & $-$3.01 & <1.64 & 0 &   1 \\
CS22963-004 &  02 56 46.6 & $-$04 51 17.5 & 5597 & 3.34 & 1.7 & $-$3.5 & $-$3.54 & 0.40 & 0 &  13 \\
CS22968-014 &  03 06 29.5 & $-$54 30 32.5 & 4864 & 1.60 & 1.9 & $-$3.6 & $-$3.58 & 0.25 & 0 &   7 \\
CS22172-002 &  03 14 20.8 & $-$10 35 11.3 & 4893 & 1.68 & 2.0 & $-$3.8 & $-$3.77 & 0.00 & 0 &   7 \\
HE0355-3728\tablenotemark{d} &  03 56 36.5 & $-$44 34 03.4 & 6418 & 4.39 & 1.4 & $-$3.4 & $-$3.41 & <2.14 & 0 &   1 \\
HE0355-3728\tablenotemark{e} &  03 56 36.5 & $-$44 34 03.4 & 6418 & 3.84 & 1.5 & $-$3.4 & $-$3.41 & <2.34 & 0 &   1 \\
CS22186-025 &  04 24 32.8 & $-$37 09 02.6 & 4871 & 1.66 & 2.0 & $-$3.1 & $-$3.07 & $-$0.54 & 0 &   7 \\
HE0557-4840 &  05 58 39.3 & $-$48 39 56.8 & 4900 & 2.20 & 1.8 & $-$4.8 & $-$4.81 & 1.65 & 1 &  15 \\
HE0945-1435\tablenotemark{d} &  09 47 50.7 & $-$14 49 06.9 & 6344 & 4.43 & 1.2 & $-$3.8 & $-$3.77 & <1.70 & 0 &   1 \\
HE0945-1435\tablenotemark{e} &  09 47 50.7 & $-$14 49 06.9 & 6344 & 3.71 & 1.4 & $-$3.8 & $-$3.78 & <1.81 & 0 &   1 \\
HE1005-1439 &  10 07 52.4 & $-$14 54 21.0 & 5202 & 2.55 & 1.6 & $-$3.1 & $-$3.09 & 2.48 & 1 &   4 \\
HE1012-1540 &  10 14 53.5 & $-$15 55 53.2 & 5745 & 3.45 & 1.4 & $-$3.5 & $-$3.47 & 2.22 & 1 &  10 \\
BS16469-075 &  10 15 10.2 & +42 53 17.3 & 4919 & 1.78 & 1.6 & $-$3.3 & $-$3.25 & 0.21 & 0 &  12 \\
HE1116-0054\tablenotemark{d} &  11 18 47.8 & $-$01 11 19.4 & 6454 & 4.37 & 1.6 & $-$3.5 & $-$3.49 & <1.72 & 0 &   1 \\
HE1116-0054\tablenotemark{e} &  11 18 47.8 & $-$01 11 19.4 & 6454 & 3.80 & 1.6 & $-$3.5 & $-$3.48 & <1.92 & 0 &   1 \\
BS16545-089 &  11 24 27.5 & +36 50 28.8 & 6486 & 3.82 & 1.4 & $-$3.4 & $-$3.44 & <1.77 & 0 &   1 \\
53436-1996-093 &  11 28 13.6 & +38 41 48.9 & 6449 & 4.38 & 1.3 & $-$3.5 & $-$3.53 & <1.66 & 0 &   1 \\
HE1150-0428 &  11 53 06.6 & $-$04 45 03.4 & 5208 & 2.54 & 1.6 & $-$3.5 & $-$3.47 & 2.37 & 1 &   9 \\
HE1201-1512\tablenotemark{d} &  12 03 37.0 & $-$15 29 33.0 & 5725 & 4.67 & 0.9 & $-$3.9 & $-$3.86 & 1.14 & 1 &   1 \\
HE1201-1512\tablenotemark{e} &  12 03 37.0 & $-$15 29 33.0 & 5725 & 3.39 & 1.5 & $-$3.9 & $-$3.92 & 1.60 & 1 &   1 \\
BS16920-017 &  12 07 16.8 & +41 39 32.5 & 4851 & 1.58 & 1.7 & $-$3.4 & $-$3.40 & $<-$0.07 & 0 &  12 \\
BS16085-050 &  12 37 46.7 & +19 22 49.5 & 4910 & 1.76 & 1.8 & $-$3.2 & $-$3.16 & $<-$0.52 & 0 &  12 \\
BS16076-006 &  12 48 22.8 & +20 56 44.0 & 5566 & 3.32 & 1.7 & $-$3.5 & $-$3.51 & 0.34 & 0 &   5 \\
HE1300+0157 &  13 02 56.2 & +01 41 52.1 & 5529 & 3.25 & 1.5 & $-$3.8 & $-$3.75 & 1.31 & 1 &  10, 11 \\
BS16929-005 &  13 03 29.5 & +33 51 09.1 & 5229 & 2.61 & 1.6 & $-$3.4 & $-$3.34 & 0.99 & 1 &   4, 12, 13 \\
HE1320-2952 &  13 22 54.9 & $-$30 08 05.3 & 5106 & 2.26 & 1.5 & $-$3.7 & $-$3.69 & <0.52 & 0 &   1 \\
HE1327-2326 &  13 30 06.0 & $-$23 41 49.7 & 6180 & 3.70 & 1.7 & $-$5.5 & $-$5.76 & 4.26 & 1 &   3 \\
BS16467-062 &  13 42 00.6 & +17 48 40.9 & 5310 & 2.80 & 1.7 & $-$3.7 & $-$3.80 & 0.40 & 0 &   7, 10, 13 \\
HE1346-0427\tablenotemark{d} &  13 49 25.1 & $-$04 42 14.8 & 6255 & 4.47 & 1.2 & $-$3.6 & $-$3.57 & <1.10 & 0 &   1 \\
HE1346-0427\tablenotemark{e} &  13 49 25.1 & $-$04 42 14.8 & 6255 & 3.69 & 1.4 & $-$3.6 & $-$3.58 & <1.31 & 0 &   1 \\
HE1347-1025 &  13 50 22.4 & $-$10 40 18.9 & 5206 & 2.52 & 1.8 & $-$3.8 & $-$3.71 & 0.15 & 0 &  10 \\
HE1356-0622 &  13 59 30.3 & $-$06 36 35.0 & 4953 & 1.85 & 1.9 & $-$3.7 & $-$3.63 & $<-$0.05 & 0 &  10 \\
HE1402-0523\tablenotemark{d} &  14 04 38.0 & $-$05 38 13.5 & 6418 & 4.38 & 1.0 & $-$3.2 & $-$3.17 & <1.50 & 0 &   1 \\
HE1402-0523\tablenotemark{e} &  14 04 38.0 & $-$05 38 13.5 & 6418 & 3.82 & 1.2 & $-$3.2 & $-$3.19 & <1.62 & 0 &   1 \\
BS16550-087 &  14 10 26.7 & +18 01 24.0 & 4754 & 1.32 & 2.2 & $-$3.6 & $-$3.54 & $-$0.49 & 0 &  13 \\
HE1424-0241 &  14 26 40.3 & $-$02 54 27.5 & 5260 & 2.66 & 1.6 & $-$4.1 & $-$4.05 & $<$0.63 & 0 &  10 \\
HD126587 &  14 27 00.4 & $-$22 14 38.9 & 4853 & 1.61 & 1.6 & $-$3.0 & $-$3.00 & 0.19 & 0 &  12 \\
BS16477-003 &  14 32 56.9 & +06 46 07.0 & 4879 & 1.66 & 1.7 & $-$3.4 & $-$3.39 & 0.29 & 0 &   7 \\
CS30325-094 &  14 54 39.3 & +04 21 38.1 & 4948 & 1.85 & 1.6 & $-$3.4 & $-$3.35 & 0.00 & 0 &   7 \\
HE1506-0113 &  15 09 14.3 & $-$01 24 56.6 & 5016 & 2.01 & 1.6 & $-$3.5 & $-$3.54 & 1.47 & 1 &   1 \\
CS30312-059 &  15 34 48.8 & $-$01 23 37.3 & 4908 & 1.75 & 1.7 & $-$3.2 & $-$3.22 & 0.27 & 0 &  13 \\
CS22884-108 &  15 49 57.6 & $-$09 14 09.2 & 6107 & 4.52 & 1.2 & $-$3.3 & $-$3.30 & $<$0.92 & 0 &  13 \\
BS16084-160 &  16 28 50.8 & +54 37 06.8 & 4727 & 1.27 & 2.0 & $-$3.2 & $-$3.20 & $-$0.12 & 0 &  13 \\
CS22878-101 &  16 45 31.4 & +08 14 45.5 & 4796 & 1.44 & 1.9 & $-$3.4 & $-$3.31 & $-$0.29 & 0 &   6,  7 \\
BS16080-093 &  16 50 38.3 & +59 13 06.5 & 4945 & 1.85 & 1.9 & $-$3.2 & $-$3.23 & $<-$0.63 & 0 &  13 \\
CS22891-209 &  19 42 02.2 & $-$61 03 44.7 & 4699 & 1.18 & 2.1 & $-$3.3 & $-$3.32 & $-$0.65 & 0 &   7 \\
BD-18 5550 &  19 58 49.7 & $-$18 12 10.9 & 4558 & 0.81 & 1.7 & $-$3.2 & $-$3.20 & $-$0.02 & 1 &   7 \\
CS22885-096 &  20 20 51.2 & $-$39 53 30.2 & 4992 & 1.93 & 1.8 & $-$3.9 & $-$3.86 & 0.26 & 0 &   7 \\
CS22950-046 &  20 21 28.4 & $-$13 16 33.6 & 4769 & 1.37 & 1.7 & $-$3.4 & $-$3.39 & \ldots & 0 &   6 \\
HE2032-5633 &  20 36 24.9 & $-$56 23 05.8 & 6457 & 3.78 & 1.8 & $-$3.6 & $-$3.63 & <2.36 & 0 &   1 \\
CS30336-049 &  20 45 23.5 & $-$28 42 35.9 & 4725 & 1.19 & 2.1 & $-$4.1 & $-$4.10 & <0.23 & 0 &   1 \\
CS22880-086 &  20 45 47.5 & $-$18 33 32.4 & 5196 & 2.54 & 1.5 & $-$3.1 & $-$3.05 & 0.24 & 0 &  13 \\
HE2047-5612 &  20 51 22.1 & $-$56 00 52.9 & 6128 & 3.68 & 0.9 & $-$3.1 & $-$3.14 & <1.37 & 0 &   1 \\
CS22897-008 &  21 03 11.9 & $-$65 05 08.8 & 4795 & 1.43 & 1.9 & $-$3.5 & $-$3.50 & 0.56 & 1 &   7 \\
CS29498-043 &  21 03 52.1 & $-$29 42 50.2 & 4639 & 1.00 & 1.7 & $-$3.5 & $-$3.49 & 1.90 & 1 &   2 \\
HE2135-1924 &  21 38 04.7 & $-$19 11 04.4 & 6449 & 4.37 & 1.2 & $-$3.3 & $-$3.31 & <1.74 & 0 &   1 \\
HE2139-5432 &  21 42 42.4 & $-$54 18 42.9 & 5416 & 3.04 & 0.8 & $-$4.0 & $-$4.02 & 2.59 & 1 &   1 \\
CS22948-066 &  21 44 51.2 & $-$37 27 55.0 & 5077 & 2.20 & 1.9 & $-$3.2 & $-$3.20 & 0.00 & 0 &   7 \\
CS22948-093 &  21 50 31.5 & $-$41 07 49.3 & 6609 & 4.23 & 1.5 & $-$3.2 & $-$3.17 & \ldots & 0 &   5 \\
CS22956-050 &  21 58 05.8 & $-$65 13 27.1 & 4844 & 1.56 & 1.8 & $-$3.4 & $-$3.39 & 0.27 & 0 &   7 \\
CS22965-054 &  22 06 30.3 & $-$02 32 34.4 & 6137 & 3.68 & 1.5 & $-$3.1 & $-$3.10 & 0.62 & 0 &   5, 13 \\
CS22892-052 &  22 17 01.7 & $-$16 39 27.1 & 4825 & 1.54 & 1.6 & $-$3.1 & $-$3.03 & 0.90 & 1 &   7, 12 \\
CS29502-042 &  22 21 48.8 & +02 28 44.9 & 5039 & 2.09 & 1.6 & $-$3.3 & $-$3.27 & 0.16 & 0 &   7 \\
CS29516-024 &  22 26 15.4 & +02 51 46.3 & 4637 & 1.04 & 1.6 & $-$3.1 & $-$3.05 & $-$0.06 & 0 &   7 \\
CS29491-053 &  22 36 56.3 & $-$28 31 06.5 & 4700 & 1.21 & 1.9 & $-$3.0 & $-$3.03 & $-$0.27 & 0 &   7 \\
CD-24 17504 &  23 07 20.2 & $-$23 52 35.6 & 6236 & 3.70 & 1.6 & $-$3.4 & $-$3.38 & \ldots & 0 &  14 \\
CS22888-031 &  23 11 32.5 & $-$35 26 42.9 & 6241 & 4.47 & 1.3 & $-$3.3 & $-$3.31 & 0.38 & 0 &   5 \\
HE2323-0256 &  23 26 29.8 & $-$02 39 57.9 & 4958 & 1.84 & 1.9 & $-$4.0 & $-$3.97 & 1.06 & 1 &   7, 10 \\
CS22966-011 &  23 35 07.0 & $-$30 22 54.4 & 6298 & 4.43 & 1.3 & $-$3.0 & $-$3.02 & 0.45 & 0 &   5 \\
CS22952-015 &  23 37 28.7 & $-$05 47 56.6 & 4824 & 1.50 & 1.9 & $-$3.5 & $-$3.44 & $-$0.41 & 0 &   7, 12 \\
HE2356-0410 &  23 59 13.1 & $-$03 53 48.2 & 5170 & 2.45 & 1.4 & $-$3.2 & $-$3.19 & 2.27 & 1 &   2,  9 \\
\enddata

\tablenotetext{a}{Coordinates are on the 2MASS system \citep{2mass}}
\tablenotetext{b}{For literature stars, [C/Fe] is the (average) value from the reference(s).}
\tablenotetext{c}{We adopt the \citet{aoki07} CEMP definition.} 
\tablenotetext{d}{This analysis assumes the star is a dwarf.} 
\tablenotetext{e}{This analysis assumes the star is a subgiant.} 

\tablerefs{
1 = This study; 
2 = \citet{aoki02}; 
3 = \citet{aoki06}; 
4 = \citet{aoki07}; 
5 = \citet{bonifacio07,bonifacio09}; 
6 = \citet{carretta02,cohen02}; 
7 = \citet{cayrel04,spite05}; 
8 = \citet{christlieb04}; 
9 = \citet{cohen06}; 
10 = \citet{cohen08}; 
11 = \citet{frebel07}; 
12 = \citet{honda04}; 
13 = \citet{lai08}; 
14 = \citet{norris01}; 
15 = \citet{norris07}
}

\end{deluxetable} 

